A Novel $p$-Harmonic Descent Approach Applied to Fluid Dynamic Shape Optimization

We introduce a novel method for the implementation of shape optimziation in fluid dynamics applications, where we propose to use the shape derivative to determine deformation fields with the help of the $p-$ Laplacian for $p > 2$. This approach is closely related to the computation of steepest descent directions of the shape functional in the $W^{1,\infty}-$ topology. Our approach is demonstrated for shape optimization related to drag-minimal free floating bodies. The method is validated against existing approaches with respect to convergence of the optimization algorithm, the obtained shape, and regarding the quality of the computational grid after large deformations. Our numerical results strongly indicate that shape optimization related to the $W^{1,\infty}$-topology -- though numerically more demanding -- seems to be superior over the classical approaches invoking Hilbert space methods, concerning the convergence, the obtained shapes and the mesh quality after large deformations, in particular when the optimal shape features sharp corners.

==> input/plaplace.tex <==
\section{$p$-Laplace Problem}
\label{sc:plaplace}
%
Since problem \eqref{eq:infinityLaplacianProblem} is numerically challenging to solve, it is approximated by the relaxation \eqref{eq:pLaplacianVariationalForm} with the minimizing function $u_p \in W^{1,p}(\Omega)$ as as approximation of the steepest descent direction $u \in W^{1,\infty}$. The minimisation problem in \eqref{eq:pLaplacianVariationalForm} is the associated variational to the $p$-Laplacian problem
%
\begin{equation}
    \begin{cases}
    - \div{\big( (\nabla u_p \colon \nabla u_p)^{\frac{p-2}{2}} \nabla u_p\big)} = 0 & \text{in} \, \Omega \\
    (\nabla u_p \colon \nabla u_p)^{\frac{p-2}{2}} \frac{\partial u_p}{\partial n} = \gamma n & \text{on} \, \Gamma \\
    u_p = 0 & \text{on} \, \partial \Omega \backslash \Gamma 
    \end{cases}
    \label{eq:plaplacianProblem}
\end{equation}
%
with $\nabla u_p \colon \nabla u_p = \sum_{i=1}^d \sum_{j=1}^d \Big( \frac{\partial u_{p,j}}{\partial x_i} \Big)^2$ and $\Gamma \subset \partial \Omega$ being that part of the boundary which is free for deformation. If $u_p \in W^{1,p}(\Omega)$ is a good approximation for the limit function $u = \lim_{p \rightarrow \infty} u_p$ with a sufficient big $p$ a displacement field for the shape optimization problem in \eqref{eq:shapeOptimisationProblem} can be obtained from \eqref{eq:plaplacianProblem} by assuming that transformations $T = \id + u_p$ with $u_p \in W^{1,p}_{0}(\Omega)$ lead to admissible domains.

%For the finite volume discretization of the $p$-Laplacian problem we refer to \cite{rung2009challenges, stuck2012adjoint, andreianov2004finite, andreianov2006finite}. 

%\paragraph{The discretization of the $p$-Laplace} is realized with a finite volume method of second order accuracy. Therefore let $\mathcal{T}$ be a partition of $\Omega \subset B$ in a way that $\Omega = \bigcup_{K \in \mathcal{T}} K$ and $K_i \cup K_j = \emptyset, \, i \neq j$. The set $\mathcal{N}_K \subset \mathcal{T}$ are the neighbor cells of $K$ with midpoints $x_N$.
%\nk{Warum muss man das so kompliziert/verschachtelt schreiben?}. \pmm{Muss man nicht aber mir fällt keine kürzere variante ein. ?}
%The corresponding midpoint of cell $K$ may be written as $x_P$ and the point $x_{PN}$ marks the point located on the centre of the face shared by two adjacent cells $K$ and $N$.
%%
%The numerical implementation follows a generic (linear) transport equation based on a cell-centered variable arrangement for the variable $u$, (cf. \cite{rung2009challenges, stuck2013adjoint, kuhl2020adjoint}), and is adopted for the (nonlinear) p-Laplace equation, viz.
%\begin{gather}
%		- \int_{K} \div{\big( \eta(u_p) \nabla u_p \big)} \, \mathrm{d} x = \nonumber \\ % - \sum_{K}\int_{K} \div{\big( \eta(u_p) \nabla u_p \big)} \, \mathrm{d} x \nonumber \\
%		%
%		%=  - \sum_{K}\int_{\partial K} \eta(u_p) \nabla u_p \cdot n \, \mathrm{d} s \nonumber \\
%		\sum_{\mathrm{faces}} \Big( \eta(u_p) \frac{\partial u_p}{\partial n} \Delta s \Big)  = 0 \quad \forall K \in .
%\end{gather}
%%
%Here, $\eta(u_p) = (\nabla u_p \colon \nabla u_p)^{(p-2)/2}$ and $\mathcal{N}_K$ refer to a non-linear diffusivity as well as the set of indices of the neighboring cells of cell $K$ respectively. A Picard linearization is employed to account for the non-linearity at iteration $k$ and the diffusive fluxes follow from the previous iteration $k-1$, i.e. $\eta(u_p^{k-1})$ as well as the face-based gradient
%%
%\begin{gather}
%		\frac{\partial u_p^k}{\partial n} (x_{PN}) 
%		\approx \frac{u_p^k(x_N) - u_p^k(x_P)}{|\Delta x_{PN}|} \nonumber \\
%		+ \nabla u_p^{k-1}(x_{PN}) \cdot \Big( n(x_{PN}) - \frac{\Delta x_{PN}}{|\Delta x_{PN}|} \Big)
%\end{gather}
%%
%where $\Delta x_{PN} = x_p - x_N$ contains a deferred correction term which contributes to the right hand side of the linear equation system. The required gradient follows from a least squares approach. The assembly of the linear equation system \nk{$A U_p = B$} for one Picard iteration is outlined in algorithm~\ref{alg::pLaplacianLinearSystemAssembly}, where $U_p \in \mathbb{R}^n$ is the discretization of $u_p$. The matrix $A \in \mathbb{R}^{n \times n}$ is a symmetric sparse matrix with diagonal elements $A_p$ and $A_N$ corresponding to the neighboring cells.
%%
%\begin{algorithm}[ht!]
%	\begin{algorithmic}
%		\State \nk{$A_P = 0$}, $A_N = 0$, \nk{$B_P=0$}
%		\ForAll{$P$}
%		\ForAll{$N$}
%		\State $\eta \gets  \big( \nabla u_p^{k-1} \colon \nabla u_p^{k-1} \big)^{(p-2)/2}$
%		\State $\Delta x_{PN} \gets x_N - x_P$
%		\State $A_N \gets \frac{\eta}{|\Delta x_{PN}|} n \Delta s $
%		\State $A_P \gets A_P - A_N$
%		\State $B_{P} \gets B_{P} - \eta \nabla u_p^{k-1} \cdot \big(n - \frac{\Delta x_{PN}}{|\Delta x_{PN}|} \big) \Delta s$
%		\EndFor
%		\EndFor
%	\end{algorithmic}
%	\caption{}
%	\label{alg::pLaplacianLinearSystemAssembly}
%\end{algorithm}
%%
%For numerical stabilisation the relaxation of the fixed point iteration is implemented as
%%
%\begin{equation}
%    A_P \gets \frac{A_P}{\omega}, \qquad B_P \gets B_P + \frac{1 - \omega}{\omega} A_p \, u_p^{k-1}(x_P)
%\end{equation}
%%
%with $\omega \in (0, 1]$. \nk{Typical values refer to ...}

%\nk{
%\paragraph{The approximation} of all PDE's follows a conventional, \nk{pressure-based}, second-order accurate finite-volume scheme based on a cell-centered variable arrangement for the variable $\phi$ located in the center of a control volume P with size $\Delta \Omega^\mathrm{P}$, e.g. \cite{rung2009challenges, stuck2013adjoint}. 
%
%Relations with adjacent control volumes NB yield one line within the discrete system, i.e. $A^\mathrm{P} \phi^\mathrm{P} - \sum_\mathrm{NB} A^\mathrm{NB} \phi^\mathrm{NB} = S_\mathrm{\phi} \Delta \Omega^\mathrm{P}$.
%
%The numerical implementation follows a generic (linear) transport equation and is adopted for the (nonlinear) p-Laplace equation
%\begin{align}
%\mu &\to \mu + ... \, \\
%A^\mathrm{P} &\to A^\mathrm{P} + \sum_\mathrm{F(P)} \left[ \mu \frac{\Delta \Gamma}{|| d_\mathrm{k}^\mathrm{F} ||} \right]^\mathrm{F}  \quad \mathrm{and} \quad \\
%S^\mathrm{P} &\to S^\mathrm{P} - \left[ \mu \frac{\partial \, \varphi}{\partial \, x_\mathrm{k}} \, \left( n_\mathrm{k} - \frac{d_\mathrm{k}}{|| d_\mathrm{k} ||} \right) \right]^\mathrm{F}
%\end{align}
%\begin{align}
%\mu \to (\nabla \tilde{u}_p \colon \nabla \tilde{u}_p)^{\frac{p-2}{2}}
%\quad \mathrm{and} \quad 
%\, , \quad 
%A^\mathrm{P} \to 
%A^\mathrm{P} + 
%\sum_\mathrm{F(P)} \left[ \mu \, \nabla u_p \right]^\mathrm{F}
%\end{align}
%where the p-Laplace diffusivity 
%is conceptually splitted into a linear/non-linear component which in turn is assembled implicitly/explicitly 
%follows from the solution $\tilde{u}_p$ of the last iteration in terms of a Picard-linearization. \nk{Mention non-orthogonality correction} Hence, the non-linearity in terms of $p > 2$ 
%serves as a source term 
%is iterated to convergence and requires under-relaxation, viz.
%\begin{align}
%A^\mathrm{P} \to \frac{A^\mathrm{P}}{\omega} 
%\quad \mathrm{and} \quad
%\, , \quad
%S^\mathrm{P} \to 
%S^\mathrm{P} + 
%\frac{\left( 1 - \omega\right) A^\mathrm{P} }{\omega} \tilde{u}_p \, . \label{equ:relaxation}
%\end{align}
%\nk{Typical values of the relaxation parameter refer to $\omega = [1.0,0.8,0.6,0.4,0.2]$ for $p = [2,3,4,5,6,]$.}
%}
